Mulitgraded Dyson-Schwinger systems

We study systems of combinatorial Dyson-Schwinger equations with an arbitrary number $N$ of coupling constants. The considered Hopf algebra of Feynman graphs is $\mathbb{N}^N$-graded, and we wonder if the graded subalgebra generated by the solution is Hopf or not. We first introduce a family of pre-Lie algebras which we classify, dually providing systems generating a Hopf subalgebra, we also describe the associated groups, as extensions of groups of formal diffeomorphisms on several variables. We then consider systems coming from Feynman graphs of a Quantum Field Theory. We show that if the number $N$ of independent coupling constants is the number of interactions of the considered QFT, then the generated subalgebra is Hopf. For QED, $\varphi^3$ and QCD, we also prove that this is the minimal value of $N$. All these examples are generalizations of the first family of Dyson-Schwinger systems in the one coupling constant case, called fundamental.We also give a generalization of the second family, called cyclic.

==> arbresbinaires.tex <==
%Arbres binaires

\newcommand{\bun}{
\begin{picture}(5,5)(-2,0)
\put(0,0){\line(0,0){5}}
\end{picture}}

\newcommand{\bdeux}{
\begin{picture}(10,15)(-5,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\end{picture}}

\newcommand{\btroisun}{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\end{picture}}
\newcommand{\btroisdeux}{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\end{picture}}

\newcommand{\bquatreun}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-9.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatredeux}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatretrois}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrequatre}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(2.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrecinq}{
\begin{picture}(15,20)(-7,0)
\put(0,0){\line(0,1){5}}
\put(0,5){\line(2,1){10}}
\put(0,5){\line(-2,1){10}}
\put(-3,6.5){\line(0,1){5}}
\put(3,6.5){\line(0,1){5}}
\end{picture}}

%Arbres binaires décorés

\newcommand{\bddeux}[1]{
\begin{picture}(25,22)(-12,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){10}}
\put(-9,7){\tiny #1}
\end{picture}}

\newcommand{\bdtroisun}[2]{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\put(-7,4){\tiny #1}
\put(-14,11){\tiny #2}
\end{picture}}

\newcommand{\bdtroisdeux}[2]{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\put(2,4){\tiny #1}
\put(9,11){\tiny #2}
\end{picture}}

\newcommand{\bddtroisun}[5]{
\begin{picture}(30,40)(-20,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){20}}
\put(-10,20){\line(1,1){10}}
\put(-9,7){\tiny #1}
\put(-19,17){\tiny #2}
\put(-21,32){\tiny #3}
\put(-1,32){\tiny #4}
\put(9,22){\tiny #5}
\end{picture}}
\newcommand{\bddtroisdeux}[5]{
\begin{picture}(30,40)(-10,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){20}}
\put(0,10){\line(-1,1){10}}
\put(10,20){\line(-1,1){10}}
\put(3,7){\tiny #1}
\put(13,17){\tiny #2}
\put(-11,22){\tiny #3}
\put(-1,32){\tiny #4}
\put(19,32){\tiny #5}
\end{picture}}


==> feynman.tex <==
\newcommand{\photonboson}{\begin{fmffile}{FEYNMAN1}\parbox{9mm}{\begin{fmfgraph}(25,25)
\fmfleft{i1}
\fmfright{o1,o2}
\fmf{photon}{i1,v}
\fmf{fermion}{o1,v,o2}
\fmfblob{.3w}{v}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\photon}{\begin{fmffile}{FEYNMAN2}\parbox{9mm}{\begin{fmfgraph}(25,25)
\fmfleft{i}
\fmfright{o}
\fmf{photon}{i,v}
\fmf{photon}{v,o}
\fmfblob{.3w}{v}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\boson}{\begin{fmffile}{FEYNMAN3}\parbox{9mm}{\begin{fmfgraph}(25,25)
\fmfleft{i}
\fmfright{o}
\fmf{fermion}{i,v}
\fmf{fermion}{v,o}
\fmfblob{.3w}{v}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\grapheun}{\begin{fmffile}{FEYNMAN4}\parbox{9mm}{\begin{fmfgraph}(28,30)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,o2}\fmf{photon}{i,v2}
\fmffreeze \fmf{photon}{v1,v3}\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphedeux}{\begin{fmffile}{FEYNMAN5}\parbox{11mm}{\begin{fmfgraph}(30,30)
\fmfleft{i}\fmfright{o}\fmf{photon}{i,v1}\fmf{photon}{v2,o}\fmf{fermion,left,tension=.2}{v1,v2,v1}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphetrois}{\begin{fmffile}{FEYNMAN6}\parbox{15mm}{\begin{fmfgraph}(40,30)
\fmfleft{i}\fmfright{o}\fmf{fermion}{i,v1,v2,o}\fmf{photon,left,tension=0. }{v1,v2}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphequatre}{\begin{fmffile}{FEYNMAN7}\parbox{18mm}{\begin{fmfgraph}(50,30)
\fmfleft{i}\fmfright{o}\fmf{photon}{i,v1}\fmf{photon}{v3,o}\fmf{fermion,tension=0.5}{v1,v2,v3,v4,v1}
\fmf{photon}{v2,v4}\fmffixed{(0,h)}{v2,v4}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphecinq}{\begin{fmffile}{FEYNMAN8}\parbox{12mm}{\begin{fmfgraph}(40,40)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v3}
\fmffreeze\fmf{photon}{v1,v5}\fmffreeze\fmf{photon}{v2,v4}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphesix}{\begin{fmffile}{FEYNMAN9}\parbox{12mm}{\begin{fmfgraph}(40,40)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v2}
\fmffreeze\fmf{photon}{v1,v4}\fmf{photon,left,tension=0.2}{v3,v5}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphesept}{\begin{fmffile}{FEYNMAN10}\parbox{12mm}{\begin{fmfgraph}(40,40)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v4}
\fmffreeze\fmf{photon,left,tension=0.2}{v1,v3}\fmffreeze\fmf{photon}{v2,v5}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphehuit}{\begin{fmffile}{FEYNMAN11}\parbox{14mm}{\begin{fmfgraph}(50,50)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v4}
\fmffreeze\fmf{photon,left,tension=0.3}{v2,v3}\fmffreeze\fmf{photon}{v1,v5}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\grapheneuf}{\begin{fmffile}{FEYNMAN12}\parbox{14mm}{\begin{fmfgraph}(50,50)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v2}
\fmffreeze\fmf{photon}{v1,v5}\fmffreeze\fmf{photon,left,tension=0.8}{v3,v4}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\graphedix}{\begin{fmffile}{FEYNMAN13}\parbox{14mm}{\begin{fmfgraph}(50,50)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1,v2,v3,v4,v5,o2}\fmf{photon}{i,v3}
\fmffreeze\fmf{photon}{v1,v4}\fmffreeze\fmf{photon}{v2,v5}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\grapheonze}{\begin{fmffile}{FEYNMAN14}\parbox{18mm}{\begin{fmfgraph}(50,50)
\fmfleft{i}\fmfright{o1,o2}\fmf{fermion}{o1,v1}\fmf{plain}{v1,w1} \fmf{fermion}{w1,v2} \fmf{plain}{v2,w2} \fmf{fermion}{w2,v3}
\fmf{fermion}{v3,o2}\fmf{photon}{i,v2}\fmffreeze\fmf{photon}{v1,v4}\fmf{photon}{v3,v5}\fmf{fermion,left,tension=0.2}{v4,v5,v4}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\arretee}{\begin{fmffile}{FEYNMAN15}\parbox{8mm}{\begin{fmfgraph}(20,20)
\fmfleft{i}\fmfright{o}\fmf{fermion}{i,o}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\arretep}{\begin{fmffile}{FEYNMAN16}\parbox{8mm}{\begin{fmfgraph}(20,20)
\fmfleft{i}\fmfright{o}\fmf{boson}{i,o}
\end{fmfgraph}}\end{fmffile}}

\newcommand{\sommet}{\begin{fmffile}{FEYNMAN17}\parbox{7mm}{\begin{fmfgraph}(20,20)
\fmfleft{i1}\fmfright{o1,o2}\fmf{boson}{i1,v}\fmf{fermion}{o1,v,o2}
\end{fmfgraph}}\end{fmffile}}
